Advanced discretization techniques for hyperelastic physics-augmented neural networks

In the present work, advanced spatial and temporal discretization techniques are tailored to hyperelastic physics-augmented neural networks, i.e., neural network based constitutive models which fulfill all relevant mechanical conditions of hyperelasticity by construction. The framework takes into account the structure of neural network-based constitutive models, in particular, that their derivatives are more complex compared to analytical models. The proposed framework allows for convenient mixed Hu-Washizu like finite element formulations applicable to nearly incompressible material behavior. The key feature of this work is a tailored energy-momentum scheme for time discretization, which allows for energy and momentum preserving dynamical simulations. Both the mixed formulation and the energy-momentum discretization are applied in finite element analysis. For this, a hyperelastic physics-augmented neural network model is calibrated to data generated with an analytical potential. In all finite element simulations, the proposed discretization techniques show excellent performance. All of this demonstrates that, from a formal point of view, neural networks are essentially mathematical functions. As such, they can be applied in numerical methods as straightforwardly as analytical constitutive models. Nevertheless, their special structure suggests to tailor advanced discretization methods, to arrive at compact mathematical formulations and convenient implementations.

==> chapter/basics.tex <==
\subsection{Hyperelasticity}
We use the analytical model
\begin{equation}
    W=a(I_1-3)+b(I_2-3)+\frac{c}{2}(J-1)^2-d\log J
\end{equation}
as the ground truth model for data generation, with the invariants of the right Cauchy-Green tensor $\bC=\bF^T\bF$
\begin{equation}
    I_1=\tr \bC,\quad I_2 = \tr \cof \bC,\quad J=\det \bF\;.
\end{equation}
We use the parameters 
\begin{equation}
    (a,b,c,d)=(831.25,166.25,10000,2327.5)\;.
\end{equation}

==> chapter/model.tex <==
\subsection{Physics augmented artificial neural network constitutive model}
\subsubsection{Artificial neural network strain energy}
In order to fulfill material symmetry, objectivity and polyconvexity, we employ (cf.\ \cite{klein2022,linden2023})
\begin{equation}\label{equation:annModel}
  \W(\I,\II,J) = \W_{\text{ANN}}(\vec{\mathcal{I}}) + \W_{\text{vol}}(J)
\end{equation}
where \(\W_{\text{ANN}}\) is modelled with a trained, physics augmented ANN with input vector
\begin{equation}
  \vec{\mathcal{I}} = (\I,\II,J,J^*)
\end{equation}
where
\begin{equation}
  J=\sqrt{C},\quad J^*=-\sqrt{C}
\end{equation}
training data is generated via an analytical strain energy density, given by (cf.\ \cite{betsch2018})
\begin{equation}\label{equation:groundTruthModel}
  \W_{\text{GT}} = a\,(\I-3) + b\,(\II-3) - \frac{c}{2}\,(J-1)^2 - d\,\log(J)
\end{equation}
where we use the parameter
\begin{equation}\label{equation:groundTruthModelParameter}
  a = 415,625;\quad b=83,125;\quad c=0;\quad d=2\,(a+2\,b) = 1163,8
\end{equation}
Note that the chosen analytical model in \eqref{equation:groundTruthModel} with parameter in \eqref{equation:groundTruthModelParameter} also serves as ground truth (GT) model in order to verify the ANN model.
Note further that training data is usually generated via experiments but is not further examined herein. 
The volumetric term \(\W_{\text{vol}}\) in \eqref{equation:annModel} is chosen as
\begin{equation}
  \W_{\text{vol}}(J) = \alpha\,(J + J^{-1} - 2)^2
\end{equation}
\subsubsection{Artificial neural network architecture}
the ANN architecture is shown for one hidden layer with eight neurons in Fig.~\ref{figure:annArchitecture}
% \begin{figure}[h!]
%   \begin{center}
%   \setlength{\figH}{0.05\textheight}
%   \setlength{\figW}{0.3\textwidth}
%   \scalebox{0.7}{\input{figures/annArchitecture2.tikz}}
%  \end{center}
%   \caption{ANN architecture for one hidden layer and eight neurons.}
%   \label{figure:annArchitecture}
% \end{figure}
with
\begin{itemize}
\item input vector \(\vec{\mathcal{I}} = (\I,\II,J,J^*)\in\mathds{R}^4\)
\item weights \(\vec{w}^1 = [w_{ij}^1]\in\mathds{R}^{4\times8}\), \(\vec{w}^2=[w_i^2]\in\mathds{R}^8\)
\item bias \(\vec{b}^1 = [b_i^1]\in\mathds{R}^8\), \(b^2\in\mathds{R}\)
\item neurons of the hidden layer with activation function, here softmax function \(\mathcal{SP}(x)\)
\end{itemize}
feed forward computations
\begin{enumerate}
\item For the input until the hidden layer a linear transformation is performed: input vector \(\vec{\mathcal{I}}\) is multiplied by weights \(\vec{w}^1\), and bias \(\vec{b}^1\) is added which yields the intermediate vector \(\vec{h}^1\in\mathds{R}^8\)
  \begin{equation}
    \vec{h}^1 = \vec{w}^1\cdot\vec{\mathcal{I}} + \vec{b}^1
  \end{equation}
\item Within the hidden layer the activation function (here: softplus) is applied in component-wise manner, such that we obtain the next intermediate vector \(\vec{h}^2\in\mathds{R}^8\) 
  \begin{equation}
    \vec{h}^2 = \mathcal{SP}(\vec{h}^1),\quad \mathcal{SP}(x) = \log(1+e^x)
  \end{equation}
and due to the properties of the chosen activation function is known as input convex neural network (ICNN)
\item The final step is the linear transformation of the output layer, yielding the output
  \begin{equation}
    y = \vec{w}^2\cdot\vec{h}^2 + b^2
  \end{equation}
  which is equivalent to a linear activation function. 
\end{enumerate}
Overall, the ANN is given by the function composition
\begin{equation}
  \W_{\text{ANN}}(\vec{\mathcal{I}}) = y\circ\vec{h}^2\circ\vec{h}^1\circ\vec{\mathcal{I}}
\end{equation}
Note that an ANN can be understood as universal approximator ('universal approximation theorem`).

Accordingly, derivatives of \(\W_{\text{ANN}}\) can be computed as usual
\begin{itemize}
\item 1st derivative
  \begin{equation}
    \partial_{\subI}\W_{\text{ANN}} = \frac{\partial y}{\partial\vec{h}^2}\cdot\frac{\vec{h}^2}{\partial\vec{h}_1}\cdot\frac{\partial\vec{h}^1}{\partial\vec{\mathcal{I}}}
  \end{equation}
  where using the derivative of the softplus function \(\partial_x\mathcal{SP}(x)=\tfrac{e^x}{1+e^x}\) we obtain 
  \begin{equation}
    \frac{\partial y}{\partial\vec{h}^2} = \vec{w}^1,\quad \frac{\partial h_i^2}{\partial h_j^1} = \delta_{ij}\,\frac{e^{h_i^1}}{1+e^{h_i^1}},\quad \frac{\partial\vec{h}^1}{\partial\vec{\mathcal{I}}} = \vec{w}^1
  \end{equation}
  Accordingly we obtain
  \begin{equation}
    \partial_{(\subI)_i}\W_{\text{ANN}} = \sum_{a=1}^8 w_a^2\,\frac{e^{h_a^1}}{1+e^{h_a^1}}\,w_{ai}^1
  \end{equation}
\item 2nd derivative, with
  \begin{equation}
    \begin{aligned}
      \partial_{(\vec{\mathcal{I}})_j}\left(\frac{e^{h_a^1}}{1+e^{h_a^1}}\right) &= \sum_{a=1}^8 \partial_{h_a^1}\left(\frac{e^{h_a^1}}{1+e^{h_a^1}}\right)\,\frac{\partial h_a^1}{\partial(\vec{\mathcal{I}})_j}\\
      &=\sum_{a=1}^8\frac{e^{h_a^1}}{(1+e^{h_a^1})^2}\,w_{aj}^1      
    \end{aligned}
  \end{equation}
    we obtain
    \begin{equation}
      \frac{\partial^2\W_{\text{ANN}}(\vec{\mathcal{I}})}{\partial(\vec{\mathcal{I}})_i\partial(\vec{\mathcal{I}})_j} = \sum_{a=1}^8 w_a^2\,\frac{e^{h_a^1}}{(1+e^{h_a^1})^2}\,w_{ai}^1\,w_{aj}^1
    \end{equation}
\end{itemize}
The derivatives are only given for the above architecture of one hidden layer.
Multiple hidden layers can be computed in a straight forward manner. 
% \subsubsection{Training of the artificial neural network}
% \begin{itemize}
% \item ground truth (GT) model
% \item experiment settings
%   \begin{itemize}
%   \item displacement driven tension loading
%   \item shear loading
%   \item ???
%   \end{itemize}
% \item tensorflow setting
%   \begin{itemize}
%   \item version and repository
%   \item strategy (overfitting, etc.)
%   \end{itemize}
% \end{itemize}
% \newpage

The overall PANN model \cite{linden2023} is given by
%
\begin{equation}
\begin{aligned}
    W(\boldsymbol{\cI})=\alpha\left[W^\text{NN}(\boldsymbol{\cI})+W^\text{stress}(J)+W^\text{energy}\right]+W^\text{growth}(J)\;.
    \end{aligned}
\end{equation}
%
We choose the additional parameter $\alpha$ so that the stress of the NN part $W^\text{NN}$ is in the order of magnitude 1. 
%
More precisely, $W^\text{NN}$ denotes an ICNN which receives the vector of invariants as input.
%
With the deformation gradient $\bF$ and the right Cauchy-Green tensor $\bC=\bF^T\bF$, we define the invariants as follows:
%
\begin{equation}
    \begin{aligned}
    I_1 &= \tr \bC\\
    I_2 &= \tr \cof \bC\\
    I_3 &= \det \bC \\
    J &= \sqrt{I_3} = \det \bF \\
    I_3^*&=-J
    \end{aligned}
\end{equation}
%
% Here, $\cof\bC=\left(\det\bC\right)\bC^{-T}$ denotes the cofactor. 
% %
% For the model implementation we need the following derivatives:
% %
% \begin{equation}
%     \begin{aligned}
%     \frac{\partial I_1}{\partial \bC}&=\bI\\
%     \frac{\partial I_2}{\partial \bC}&=I_1\bI-\bC \\
%     \frac{\partial J}{\partial \bC}&=\frac{J}{2}\bC^{-1}\\
%     \frac{\partial I_3^*}{\partial \bC}&=-\frac{J}{2}\bC^{-1}\;.
%     \end{aligned}
% \end{equation}
%
The vector of invariants we pass to the ICNN is then given as
%
\begin{equation}
    \boldsymbol{\mathcal{I}}=\left(I_1,I_2,J,-J\right)\;.
\end{equation}
%
Then, the volumetric growth term is choosen as the analytical polyconvex term
%
\begin{equation}
    W^\text{growth}(J):=\left(J+\frac{1}{J}-2\right)^2\;.
\end{equation}
%
Then, the stress normalization term is given by
%
\begin{equation}
    W^\text{stress}(J):=-A(J-1)\;,
\end{equation}
%
where the constant
%
\begin{equation}
    A:=2\left(\frac{\partial W^\text{NN}}{\partial I_1} 
    + 2\frac{\partial W^\text{NN}}{\partial I_2} +\frac{1}{2} \frac{\partial W^\text{NN}}{\partial J}  -\frac{1}{2}\frac{\partial W^\text{NN}}{\partial I_3^*}  
    \right)\Bigg\rvert_{\bC=\bI}\in\bbR
\end{equation}
%
is a weighted sum of derivatives of the ICNN potential with respect to the invariants for the undeformed state $\bC=\bI$. The stress correction term preserves polyconvexity as it is linear in $J$. The energy normalization term is given by
%
\begin{equation}
    W^\text{energy}:=-W^\text{NN}\Bigg\rvert_{\bC=\bI}\in\bbR\,.
\end{equation}
%
This is basically the bias of the output layer.
%
Overall, the corresponding stress of the model is given by
%
\begin{equation}
    \bS=\bS^\text{NN}+\bS^\text{growth}+\bS^\text{stress}
\end{equation}
%
with
%
\begin{equation}
    \bS^\text{NN}=2\left(\frac{\partial W^\text{NN}}{\partial I_1} \bI
    + \frac{\partial W^\text{NN}}{\partial I_2}\left( I_1 \bI - \bC\right) + \frac{\partial W^\text{NN}}{\partial J} \frac{J}{2}\bC^{-1} -\frac{\partial W^\text{NN}}{\partial I_3^*}  \frac{J}{2}\bC^{-1}\right)
\end{equation}
%
\begin{equation}
    \bS^\text{growth}=2\left(J+\frac{1}{J}-2\right)\left(1-\frac{1}{J^2}\right)J\bC^{-1}
\end{equation}
%
\begin{equation}
    \bS^\text{stress}=-AJ\bC^{-1}
\end{equation}
%
Note that the energy correction term $W^\text{energy}$ is a constant, and thus does not contribute to the stress.

\medskip

At the identity $\bF=\bI$, the following holds:
%
\begin{equation}
    \begin{aligned}
    \bC=\bI,
    \quad
    \cof \bC = \bI,
    \\
    I_1=3,
    \quad
    I_3=J=1,
    \end{aligned}
\end{equation}
%
which implies
%
\begin{equation}
        \bS^\text{NN}\Big\rvert_{\bC=\bI}=2\left(\frac{\partial W^\text{NN}}{\partial I_1} 
    + 2\frac{\partial W^\text{NN}}{\partial I_2}+ \frac{1}{2}\frac{\partial W^\text{NN}}{\partial J}  -\frac{1}{2}\frac{\partial W^\text{NN}}{\partial I_3^*}  \right)\bI
\end{equation}
%
\begin{equation}
     \bS^\text{growth}\Big\rvert_{\bC=\bI}=\boldsymbol{0}
\end{equation}
%
\begin{equation}
     \bS^\text{stress}\Big\rvert_{\bC=\bI}=-A\bI
\end{equation}
%
Thus, the stress normalization is clearly fulfilled.


